Dataset and Benchmarking of Real-Time Embedded Object Detection for RoboCup SSL

When producing a model to object detection in a specific context, the first obstacle is to have a dataset labeling the desired classes. In RoboCup, some leagues already have more than one dataset to train and evaluate a model. However, in the Small Size League (SSL), there is not such dataset available yet. This paper presents an open-source dataset to be used as a benchmark for real-time object detection in SSL. This work also presented a pipeline to train, deploy, and evaluate Convolutional Neural Networks (CNNs) models in a low-power embedded system. This pipeline was used to evaluate the proposed dataset with state-of-art optimized models. In this dataset, the MobileNet SSD v1 achieves 44.88% AP (68.81% AP50) at 94 Frames Per Second (FPS) while running on an SSL robot.

==> figures/environment/v2020.tex <==
\begin{figure}[ht]
\centering
\includegraphics[width=.7\textwidth]{figures/environment/res/v2020.png}
\caption{Unmodified RobôCIn's \gls{ssl} robot v2020.}
\label{fig:robo}
\end{figure} 

==> tables/dataset/info.tex <==
\begin{table}
\centering
\caption{Instance division per class and size. Small objects have less than $32^2~(1024)$ pixels, medium objects have a size between $32^2~(1024)$ pixels and $96^2~(9216)$ pixels, and large objects are bigger than $96^2~(9216)$ pixels.}
\label{tab:dataset_info}
\begin{tabular}{p{0.19\textwidth}>{\centering}p{0.19\textwidth}>{\centering}p{0.19\textwidth}>{\centering}p{0.19\textwidth}>{\centering\arraybackslash}p{0.19\textwidth}}
\hline
\multirow{2}{*}{\textbf{Object Class}}&\multicolumn{3}{c}{\textbf{Object Size}}&\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Instances\\ per Class\end{tabular}}}\\\cline{2-4}
& \textbf{Small} & \textbf{Medium} & \textbf{Large}&\\
\hline
\textbf{Robot}                         & 1203     & 647       & 36       & 1886                   \\
\textbf{Ball}                          & 1654     & 57        & 0        & 1711                   \\
\textbf{Goal}                          & 62       & 521       & 2        & 585                    \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Instances\\per Size\end{tabular}}                         & 2919     & 1225      & 38       & 4182                   \\ 
\hline
\end{tabular}
\end{table}

==> tables/models/mobilenet_data.tex <==
\begin{table}
\centering
\caption{Hyperparameters modifications on MobileNet SSD v1, MobileNet SSD v2 and MobileDet models.}
\label{tab:models_mobilenet_data}
\begin{tabular}{p{0.4\textwidth}p{0.4\textwidth}}
\hline
\textbf{Hyperparameter} &\textbf{Used Values} \cr
\hline
\textbf{Input Size}                          & $224\times224$ \cr
\textbf{Batch Size}                           & $32$ \cr
\textbf{Data Augmentation}                           & Horizontal Flip, Image Crop, Image Scale, Brightness Adjustment, Contrast Adjustment, Saturation Adjustment, and Black Patches  \cr 
\hline
\end{tabular}
\end{table}


==> tables/results/pascal.tex <==
\begin{table}
\centering
\caption{}
\label{tab:results_pascal}
\begin{tabular}{p{0.22\textwidth}>{\centering}p{0.135\textwidth}>{\centering}p{0.135\textwidth}>{\centering}p{0.135\textwidth}>{\centering}p{0.135\textwidth}>{\centering}p{0.135\textwidth}}
\hline
\textbf{Method}&\textbf{FPS}&\textbf{mAP}&\textbf{AP$_{robot}$}&\textbf{AP$_{goal}$}&\textbf{AP$_{ball}$} \cr
\hline
\textbf{MobileDet}    & $87$ & $67.05\%$ & $63.77\%$ & $62.04\%$ & $75.36\%$ \cr
\textbf{MobileNet SSD v1} & $94$ & $69.77\%$ & $66.96\%$ & $58.33\%$ & $84.01\%$ \cr
\textbf{MobileNet SSD v2} & $78$ & $75.96\%$ & $70.80\%$ & $67.29\%$ & $89.79\%$ \cr
\textbf{YOLOv4 Tiny}  & $10$ & $62.61\%$ & $80.45\%$ & $89.54\%$ & $17.84\%$ \cr
\hline
\end{tabular}
\end{table}
